Deep or Simple Models for Semantic Tagging? It Depends on your Data [Experiments]

Semantic tagging, which has extensive applications in text mining, predicts whether a given piece of text conveys the meaning of a given semantic tag. The problem of semantic tagging is largely solved with supervised learning and today, deep learning models are widely perceived to be better for semantic tagging. However, there is no comprehensive study supporting the popular belief. Practitioners often have to train different types of models for each semantic tagging task to identify the best model. This process is both expensive and inefficient. We embark on a systematic study to investigate the following question: Are deep models the best performing model for all semantic tagging tasks? To answer this question, we compare deep models against "simple models" over datasets with varying characteristics. Specifically, we select three prevalent deep models (i.e. CNN, LSTM, and BERT) and two simple models (i.e. LR and SVM), and compare their performance on the semantic tagging task over 21 datasets. Results show that the size, the label ratio, and the label cleanliness of a dataset significantly impact the quality of semantic tagging. Simple models achieve similar tagging quality to deep models on large datasets, but the runtime of simple models is much shorter. Moreover, simple models can achieve better tagging quality than deep models when targeting datasets show worse label cleanliness and/or more severe imbalance. Based on these findings, our study can systematically guide practitioners in selecting the right learning model for their semantic tagging task.

==> def_suggestion.tex <==
\subsection{Suggestion}

% suggestion definition
Reviewers commonly provide suggestions in their comments. Based on their actual experiences and feelings, they gave constructive plans that can enhance customer satisfaction. Useful suggestions are deemed explicitly actionable []. They directly expressed actions that are easy to follow. For example, a hotel review may recommend visiting a nearby attraction for beautiful scenery or going to a local canteen for delicious food. Besides plans that encourage actions, some suggestions try to avoid negative feelings.   One such example may be a warning to females that it is not safe to walk alone on the street late at night. 

Sapna et. al.~\cite{NegiB15emnlp} asked human annotators to label explicit customer-to-customer suggestions and provided two guidelines. First, a suggestion sentence must explicitly state the intention of giving an recommendation. Second, the suggestion should have the potential benefiting customers. For example, a suggestion sentence may look like 'Try the cup cakes at the bakery next door'. An opposite example would look like "the cup cakes from the bakery next door were delicious" as it does not indicate the suggestion explicitly. 

Since suggestion expressing sentences contain great value, extracting these sentences becomes an important task for SEMEVAL competition in 2019 []. In this task, the participants were asked to build classifiers to accurately predict whether a sentence is a suggestion or not. The task also provided 9092 and 808 labeled sentences in software and hotel domain correspondingly. The best performing algorithm [] adopted the recent pre-trained BERT model that is believed to work decently with small number of training data. 

\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{|l|p{0.8\linewidth}|}
\hline
City  & Tips  \\ 
\hline
\multirow{2}{*}{Washington DC} & 1. 20\% tip is customary for most services \\
  & 2. Avoid walking through parks at night \\
\hline

\multirow{2}{*}{Hong Kong} & 1. Many 'local' restaurants offer menus in English. Ask if they have one before you sit down. \\ 
  & 2. Grab an Octopus Card to store money and use on buses, trains and in convenience stores (you have to pay deposit). It will save you a lot of time queuing or fishing for change. \\
\hline
            
\end{tabular}
}
\caption{TripAdvisor city guide tips}
\label{table:tripadvisor_tip}
\end{table}

\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{|l|p{0.8\linewidth}|}
\hline
Business  & Tips  \\ 
\hline
\multirow{2}{*}{Restaurant} & 1. There aren't many sushi choices in Mountain View, so take what you can get. \\
 & 2. Free Parking in the lot across the street and around the residential areas. \\
\hline

\multirow{2}{*}{Coffee shop} & 1. only place in Bay Area I've been able to find soft boiled eggs \\ 
  & 2. Delightful cafe with solid pastries. Drinks left more to be desired and service is abit slow, so make sure you have ample time!. \\
\hline
            
\end{tabular}
}
\caption{Yelp tips}
\label{table:yelp_tip}
\end{table}

==> designs.tex <==
\begin{table*}[!h]
\scalebox{0.8}{
\begin{tabular}{|l|l|l|l|}
\hline
  & Paper  & Input    &Output  \\
\hline
\multirow{7}{*}{Suggestion}& Suggestion dataset~\cite{NegiRB18corr} & Review sentences, human labelers & Labeled suggestions \\
                          & Semi-supervised C2C suggestion mining~\cite{GolchhaGEB18corr} & Labeled suggestions, unlabeled suggestions & semi-supervised model \\
                          & Travel tips~\cite{GuyMNR17www}   & TriAdvisor (labeled) & model in travel domain \\
                          & A Survey on suggestion mining~\cite{NegiAMB16starsem} & labeled datasets, models & comparisons of different models  \\
                          & customer-to-customer suggestion extraction~\cite{NegiB15emnlp} & labeled suggestions & SVM model\\
                          & CNN for sentence classification~\cite{Kim14emnlp} & labeled sentences & CNN model \\

\hline                     
\multirow{5}{*}{Tip}  & Unsupervised tip-mining~\cite{ZhuLZ18dss} & unlabeled review data & tip sentences  \\
                     & Reason mining~\cite{KimH06acl} & Labeled dataset &  Maximum Entropy Classification Model\\
                     & Mining product defects and improvements~\cite{Moghaddam15ecir}       & noisy dataset & SVM model (prediction), LDA model (clustering)         \\
                     & LDA based product defect mining~\cite{QiaoZZWF17hicss}               & labeled dataset & LDA model \\
                     & Mining product failure by distant supervision~\cite{Tutubalina16kesw} & different algorithms, noisy data & performance comparison\\
                     & Detecting experience from weblogs~\cite{ParkJM10acl}             & labeled sentences & LR or SVM models                       \\
\hline
\end{tabular}
}
\caption{}
\label{table:designs}
\end{table*}

% two questions
% q1: Do we need all different techniques, or we have a general solution
% q2: Can we combine all different techniques and integrate their strengths
% q3: Dependencies/tradeoff of different methods 
% q4: factorization and propose conceptual frameworks

==> discussion.tex <==
\section{Discussion} 
% process suggestions, facts and answer as sentiments
% unsupervised algorithms
Compared with extensive works on sentiment analysis, research on suggestion, fact, and answer is still at its infant. Many problems and their solutions remain unexplored. Here we list three such problems.   
\begin{itemize}
    \item Personalization. Existing applications do not consider user preferences. They display the same set of sentences to all users. However, data labeling shows that people often disagree with each other due to subjectivity. For example, a sentence may look funny to specific users, but a waste of time for others. We may consider personalization when deploying an application and develop supports such as query interfaces or user preference prediction. 
    
    \item Aspect-based analysis. Aspect-based analysis would help organize extracted sentences according to their targets. For example, we may organize all the hotel descriptions on room uncleanliness, such that the user can have a complete picture on such uncleanliness and decide whether he will accept these facts as a trade off of other benefits(e.g. price or location). 

\end{itemize}

\noindent\textbf{What constitutes a high F1.} 
% fundamental problem in a dataset: all dataset suffer from data in sufficiency
% noise: ambiguity 
%ratio (good start point)
    % formular indication
    % improve the coverage of a dataset
    % noise countering
%larger dataset due to high coverage of the vocabulary (confirmed both 20% based and 10% based)
%separability (distinct P words under same number of vocabulary)
%transferred knowledge (compensate small datasets) BERT
%domain knowledge


\noindent\textbf{How to choose a classifier}
% cost is not a concern, BERT
% cost is a concern
\noindent\textbf{All datasets suffer from label insufficiency. Most datasets suffer from label sparsity. A good model best captures the aboves}

We summarize the strengths and weaknesses of the three methods.

==> extraction.tex <==
%\section{What techniques have people explored in their solutions}

\begin{table*}[t]
\scalebox{0.8}{
\begin{tabular}{|l|l|l|l|}
\hline
    & Paper & Description\\
\hline
\multirow{2}{*}{Suggestion}& Suggestion dataset~\cite{NegiRB18corr}      & Provide a human-labeled dataset \\
                          & Semi-supervised C2C suggestion mining~\cite{GolchhaGEB18corr} & Claim the better performance (the state-of-the-art is LSTM + Attention)  \\
\hline          
\multirow{2}{*}{Humor}& Humor Recognition and Humor Anchor Extraction (CMU EMNLP 15)&  \\
                          & yelp\_funny humor (EMNLP 17) &  \\
                          & word association (COLNG 18) &  \\
                          & russian dataset (ACL 19 short) &  \\
                          & english pun (NAACL 19 short) &  \\      
                          & A Neural Approach to Pun Generation (ACL 18)& \\
                          & Semeval2017task & two tasks, detecting puns and humor tweets correspondingly \\
                          
\hline
\end{tabular}
}
\caption{}
\label{table:papersummary}
\end{table*}

\section{Automatic extraction} 
% works for different settings
%\subsection{Problem Definition}
The problem of extracting suggestions, facts or answers can be formulated as sentences classification. The input is one sentence or multiple sentences, and the output is the probability of this input satisfying the pre-defined purpose. For example, a purpose in mining suggestions would be whether the given sentence expresses customer to customer suggestions. Since the judgements of suggestions, facts and answers are subjective, existing papers usually adopt supervised learning that requires human-labeled datasets. 


There is no an objective definition of suggestion in existing works. To understand what sentences are deemed as suggestions, existing papers rely on human annotators and ask them to label a set of sentences they think are suggestions. The labeling is subjective, which depends on personal experience. Thus human annotators often diverge when labeling the same sentence and generate significant disagreement. On the other hand, the labeled sentences are domain specific. They can not fully represent the set of suggestion sentences for datasets from different domains. An application in a new domain may have to relabel its datasets.


\subsection{Rules}
Di et. al.~\cite{ZhuLZ18dss} proposes to identifying suggestion sentences without human annotated data. They proposes the concept of informative tokens, which are words or phrases used to sketch one entity. Informative tokens for an entity were selected based on their appearance. They should appear more frequently in the review commenting that entity than the reviews commenting similar entities. This paper only consider four type of words or phrases as informative tokens. They are named entities such as White House, compound n-grams such as ``street noise``, adjective-modified nouns such as ``great service`` and singleton nouns such as ``bathroom`` that satisfies predefined frequency bounds. After obtaining informative tokens for an entity, they greedily extract sentences containing the maximum number of informative tokens as tips.


% extraction techniques
%\textbf{Generate product description} eBay applied this to product review, as some sellers just post new products while they do not have time to write a complete product description. They firstly removed short sentences consisting of less than 3 words, which are unlikely to provide useful information. They also removed sentences containing personal pronouns such as "i", "my" and "our". The purpose is to avoid personal stories and make the description more objective and generally useful. In addition, they removed sentences talking about price, shipping and warranty as they want the information is about the product itself. After the removing unnecessary sentences, they asked human annotates to annotate a set of sentences by whether a sentence is suitable for product description. Negative examples include subjective comments or incomplete sentences whose meaning is not understandable without the last or next sentence. When they collected 25k labeled sentences, they build a classifier with multi-task LSTM that achieves a satisfactory prediction. They deployed this classifier to actual data and used k-means to select the set of sentences differ from each other. They run LexRank to ranked selected sentences and show high ranked sentences as final descriptions. They showed LexRank achieve the best satisfaction according to their user study. Example~\ref{eg:prodep} shows the description for a socks product. 

\subsection{Supervised learning}
Given a set of tip sentences, try to develop a supervised model for prediction. 

\subsection{Word embedding}

\subsection{Sentence embedding}
%aggregation of word embeddings into sentence embedding

\subsection{Model}

\subsection{Pre-train}

\subsection{Fine-tune}

\subsubsection{Rule Discovery}
% Our rules cover the majority existing rules
Unfortunately, existing methods 
\subsection{Weakly supervised learning}

\subsection{Other tasks}

\subsubsection{Deduplication}

\subsection{Ranking}


==> relatedwork.tex <==
\section{Related Work}
\subsection{Rule based extraction}

\subsection{Machine learning extraction}

\subsection{Neural Network extraction}


==> tmp_note.tex <==
main results
1. consider DL in production
2. evaluate tradeoff of different DL solutions in interesting sentences extraction
3. insights
strong points

weak points
1. Groundtruth is subjective
